QUBIC V: Cryogenic system design and performance

Current experiments aimed at measuring the polarization of the Cosmic Microwave Background (CMB) use cryogenic detector arrays and cold optical systems to boost the mapping speed of the sky survey. For these reasons, large volume cryogenic systems, with large optical windows, working continuously for years, are needed. Here we report on the cryogenic system of the QUBIC (Q and U Bolometric Interferometer for Cosmology) experiment: we describe its design, fabrication, experimental optimization and validation in the Technological Demonstrator configuration. The QUBIC cryogenic system is based on a large volume cryostat, using two pulse-tube refrigerators to cool at ~3K a large (~1 m^3) volume, heavy (~165kg) instrument, including the cryogenic polarization modulator, the corrugated feedhorns array, and the lower temperature stages; a 4He evaporator cooling at ~1K the interferometer beam combiner; a 3He evaporator cooling at ~0.3K the focal-plane detector arrays. The cryogenic system has been tested and validated for more than 6 months of continuous operation. The detector arrays have reached a stable operating temperature of 0.33K, while the polarization modulator has been operated from a ~10K base temperature. The system has been tilted to cover the boresight elevation range 20 deg -90 deg without significant temperature variations. The instrument is now ready for deployment to the high Argentinean Andes.

==> authors.tex <==
% authors.tex :  this file automatically generated by author_list.py
%% DO NOT EDIT.  It will be clobbered next time you run author_list.py
\author[1,2]{S.~Masi}
\author[1,2]{E.S.~Battistelli}
\author[1,2]{P.~de~Bernardis}
\author[3]{C.~Chapron}
\author[1,2]{F.~Columbro}
\author[1,2]{G.~D'Alessandro}
\author[1,2]{M.~De~Petris}
\author[3]{L.~Grandsire}
\author[3]{J.-Ch.~Hamilton}
\author[4]{S.~Marnieros}
\author[1,2]{L.~Mele}
\author[5]{A.~May}
\author[6,7]{A.~Mennella}
\author[8]{C.~O'Sullivan}
\author[1,2]{A.~Paiella}
\author[1,2]{F.~Piacentini}
\author[3]{M.~Piat}
\author[5]{L.~Piccirillo}
\author[1,2]{G.~Presta}
\author[1,9]{A.~Schillaci}
\author[10]{A.~Tartari}
\author[3]{J.-P.~Thermeau}
\author[3,11]{S.A.~Torchinsky}
\author[3]{F.~Voisin}
\author[12,13]{M.~Zannoni}
\author[14]{P.~Ade}
\author[15]{J.G.~Alberro}
\author[16]{A.~Almela}
\author[1]{G.~Amico}
\author[17]{L.H.~Arnaldi}
\author[4]{D.~Auguste}
\author[18]{J.~Aumont}
\author[19]{S.~Azzoni}
\author[12,13]{S.~Banfi}
\author[20]{B.~B\a'{e}lier}
\author[12,13]{A.~Ba\a`{u}}
\author[8]{D.~Bennett}
\author[4]{L.~Berg\a'{e}}
\author[18]{J.-Ph.~Bernard}
\author[6,7]{M.~Bersanelli}
\author[3]{M.-A.~Bigot-Sazy}
\author[21]{J.~Bonaparte}
\author[4]{J.~Bonis}
\author[22]{E.~Bunn}
\author[8]{D.~Burke}
\author[1]{D.~Buzi}
\author[6,7]{F.~Cavaliere}
\author[3]{P.~Chanial}
\author[3]{R.~Charlassier}
\author[16]{A.C.~Cobos~Cerutti}
\author[1,2]{A.~Coppolecchia}
\author[23,24]{G.~De~Gasperis}
\author[1,25]{M.~De~Leo}
\author[3]{S.~Dheilly}
\author[16]{C.~Duca}
\author[4]{L.~Dumoulin}
\author[16]{A.~Etchegoyen}
\author[21]{A.~Fasciszewski}
\author[16]{L.P.~Ferreyro}
\author[16]{D.~Fracchia}
\author[6,7]{C.~Franceschet}
\author[26]{M.M.~Gamboa Lerena}
\author[3]{K.M.~Ganga}
\author[16]{B.~Garc\a'{i}a}
\author[16]{M.E.~Garc\a'{i}a Redondo}
\author[4]{M.~Gaspard}
\author[8]{D.~Gayer}
\author[12,13]{M.~Gervasi}
\author[18]{M.~Giard}
\author[1,5]{V.~Gilles}
\author[3]{Y.~Giraud-Heraud}
\author[17]{M.~G\a'{o}mez Berisso}
\author[17]{M.~Gonz\a'{a}lez}
\author[8]{M.~Gradziel}
\author[16]{M.R.~Hampel}
\author[17]{D.~Harari}
\author[4]{S.~Henrot-Versill\a'{e}}
\author[6,7]{F.~Incardona}
\author[4]{E.~Jules}
\author[3]{J.~Kaplan}
\author[27]{C.~Kristukat}
\author[1,2]{L.~Lamagna}
\author[3,28]{S.~Loucatos}
\author[4]{T.~Louis}
\author[29]{B.~Maffei}
\author[18]{W.~Marty}
\author[2]{A.~Mattei}
\author[5]{M.~McCulloch}
\author[16]{D.~Melo}
\author[18]{L.~Montier}
\author[3]{L.~Mousset}
\author[15]{L.M.~Mundo}
\author[8]{J.A.~Murphy}
\author[8]{J.D.~Murphy}
\author[12,13]{F.~Nati}
\author[4]{E.~Olivieri}
\author[4]{C.~Oriol}
\author[18]{F.~Pajot}
\author[12,13]{A.~Passerini}
\author[17]{H.~Pastoriza}
\author[2]{A.~Pelosi}
\author[3]{C.~Perbost}
\author[2]{M.~Perciballi}
\author[6,7]{F.~Pezzotta}
\author[14]{G.~Pisano}
\author[16]{M.~Platino}
\author[1,30]{G.~Polenta}
\author[3]{D.~Pr\a^{e}le}
\author[1,31]{R.~Puddu}
\author[18]{D.~Rambaud}
\author[32]{E.~Rasztocky}
\author[15]{P.~Ringegni}
\author[32]{G.E.~Romero}
\author[16]{J.M.~Salum}
\author[26,33]{C.G.~Sc\a'{o}ccola}
\author[8,34]{S.~Scully}
\author[12]{S.~Spinelli}
\author[3]{G.~Stankowiak}
\author[3]{M.~Stolpovskiy}
\author[16]{A.D.~Supanitsky}
\author[35]{P.~Timbie}
\author[6,7]{M.~Tomasi}
\author[36]{G.~Tucker}
\author[14]{C.~Tucker}
\author[6,7]{D.~Vigan\a`{o}}
\author[23]{N.~Vittorio}
\author[4]{F.~Wicek}
\author[5]{M.~Wright}
\author[2]{and A.~Zullo}


\affiliation[1]{Universit\a`{a} di Roma - La Sapienza, Roma, Italy}
\affiliation[2]{INFN sezione di Roma, 00185 Roma, Italy}
\affiliation[3]{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France}
\affiliation[4]{Laboratoire de Physique des 2 Infinis Ir\a`{e}ne Joliot-Curie (CNRS-IN2P3, Universit\a'e Paris-Saclay), France}
\affiliation[5]{University of Manchester, UK}
\affiliation[6]{Universita degli studi di Milano, Milano, Italy}
\affiliation[7]{INFN sezione di Milano, 20133 Milano, Italy}
\affiliation[8]{National University of Ireland, Maynooth, Ireland}
\affiliation[9]{California Institute of Technology, USA}
\affiliation[10]{INFN sezione di Pisa, 56127 Pisa, Italy}
\affiliation[11]{Observatoire de Paris, Universit\'e Paris Science et Lettres, F-75014 Paris, France}
\affiliation[12]{Universit\a`{a} di Milano - Bicocca, Milano, Italy}
\affiliation[13]{INFN sezione di Milano - Bicocca, 20216 Milano, Italy}
\affiliation[14]{Cardiff University, UK}
\affiliation[15]{GEMA (Universidad Nacional de La Plata), Argentina}
\affiliation[16]{Instituto de Tecnolog\a'{i}as en Detecci\a'{o}n y Astropart\a'{i}culas  (CNEA, CONICET, UNSAM), Argentina}
\affiliation[17]{Centro At\a'{o}mico Bariloche and Instituto Balseiro (CNEA), Argentina}
\affiliation[18]{Institut de Recherche en Astrophysique et Plan\a'{e}tologie, Toulouse (CNRS-INSU), France}
\affiliation[19]{Department of Physics, University of Oxford, UK}
\affiliation[20]{Centre de Nanosciences et de Nanotechnologies, Orsay, France}
\affiliation[21]{Centro At\a'{o}mico Constituyentes (CNEA), Argentina}
\affiliation[22]{University of Richmond, Richmond, USA}
\affiliation[23]{Universit\a`{a} di Roma ``Tor Vergata'', Roma, Italy}
\affiliation[24]{INFN sezione di Roma2, 00133 Roma, Italy}
\affiliation[25]{University of Surrey, UK}
\affiliation[26]{Facultad de Ciencias Astron\a'{o}micas y Geof\a'{i}sicas (Universidad Nacional de La Plata), Argentina}
\affiliation[27]{Escuela de Ciencia y Tecnolog\a'{i}a (UNSAM) and Centro At\a'{o}mico Constituyentes (CNEA), Argentina}
\affiliation[28]{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affiliation[29]{Institut d'Astrophysique Spatiale, Orsay (CNRS-INSU), France}
\affiliation[30]{Italian Space Agency, Roma, Italy}
\affiliation[31]{Pontificia Universidad Catolica de Chile, Chile}
\affiliation[32]{Instituto Argentino de Radioastronom\a'{i}a (CONICET, CIC, UNLP), Argentina}
\affiliation[33]{CONICET, Argentina}
\affiliation[34]{Institute of Technology, Carlow, Ireland}
\affiliation[35]{University of Wisconsin, Madison, USA}
\affiliation[36]{Brown University, Providence, USA}

\emailAdd{silvia.masi@roma1.infn.it}

==> authors_5.tex <==
% authors.tex :  this file automatically generated by author_list.py
%% DO NOT EDIT.  It will be clobbered next time you run author_list.py
\author[1,2]{S.~Masi}
\author[1,2]{E.S.~Battistelli}
\author[1,2]{P.~de~Bernardis}
\author[3]{C.~Chapron}
\author[1,2]{F.~Columbro}
\author[1,2]{G.~D'Alessandro}
\author[1,2]{M.~De~Petris}
\author[3]{L.~Grandsire}
\author[3]{J.-Ch.~Hamilton}
\author[4]{S.~Marnieros}
\author[1,2]{L.~Mele}
\author[5]{A.~May}
\author[6,7]{A.~Mennella}
\author[8]{C.~O'Sullivan}
\author[1,2]{A.~Paiella}
\author[1,2]{F.~Piacentini}
\author[3]{M.~Piat}
\author[5]{L.~Piccirillo}
\author[1,2]{G.~Presta}
\author[1,9]{A.~Schillaci}
\author[10]{A.~Tartari}
\author[3]{J.-P.~Thermeau}
\author[3,11]{S.A.~Torchinsky}
\author[3]{F.~Voisin}
\author[12,13]{M.~Zannoni}
\author[14]{P.~Ade}
\author[15]{J.G.~Alberro}
\author[16]{A.~Almela}
\author[1]{G.~Amico}
\author[17]{L.H.~Arnaldi}
\author[4]{D.~Auguste}
\author[18]{J.~Aumont}
\author[19]{S.~Azzoni}
\author[12,13]{S.~Banfi}
\author[12,13]{A.~Ba\a`{u}}
\author[20]{B.~B\a'{e}lier}
\author[8]{D.~Bennett}
\author[4]{L.~Berg\a'{e}}
\author[18]{J.-Ph.~Bernard}
\author[6,7]{M.~Bersanelli}
\author[3]{M.-A.~Bigot-Sazy}
\author[21]{J.~Bonaparte}
\author[4]{J.~Bonis}
\author[22]{E.~Bunn}
\author[8]{D.~Burke}
\author[1]{D.~Buzi}
\author[6,7]{F.~Cavaliere}
\author[3]{P.~Chanial}
\author[3]{R.~Charlassier}
\author[16]{A.C.~Cobos~Cerutti}
\author[1,2]{A.~Coppolecchia}
\author[23,24]{G.~De~Gasperis}
\author[1,25]{M.~De~Leo}
\author[3]{S.~Dheilly}
\author[16]{C.~Duca}
\author[4]{L.~Dumoulin}
\author[16]{A.~Etchegoyen}
\author[21]{A.~Fasciszewski}
\author[16]{L.P.~Ferreyro}
\author[16]{D.~Fracchia}
\author[6,7]{C.~Franceschet}
\author[26,27]{M.M.~Gamboa Lerena}
\author[3]{K.M.~Ganga}
\author[16]{B.~Garc\a'{i}a}
\author[16]{M.E.~Garc\a'{i}a Redondo}
\author[4]{M.~Gaspard}
\author[8]{D.~Gayer}
\author[12,13]{M.~Gervasi}
\author[18]{M.~Giard}
\author[1,5]{V.~Gilles}
\author[3]{Y.~Giraud-Heraud}
\author[17]{M.~G\a'{o}mez Berisso}
\author[17]{M.~Gonz\a'{a}lez}
\author[8]{M.~Gradziel}
\author[16]{M.R.~Hampel}
\author[17]{D.~Harari}
\author[4]{S.~Henrot-Versill\a'{e}}
\author[6,7]{F.~Incardona}
\author[4]{E.~Jules}
\author[3]{J.~Kaplan}
\author[28]{C.~Kristukat}
\author[1,2]{L.~Lamagna}
\author[3,29]{S.~Loucatos}
\author[4]{T.~Louis}
\author[30]{B.~Maffei}
\author[18]{W.~Marty}
\author[2]{A.~Mattei}
\author[5]{M.~McCulloch}
\author[16]{D.~Melo}
\author[18]{L.~Montier}
\author[3]{L.~Mousset}
\author[15]{L.M.~Mundo}
\author[8]{J.A.~Murphy}
\author[8]{J.D.~Murphy}
\author[12,13]{F.~Nati}
\author[4]{E.~Olivieri}
\author[4]{C.~Oriol}
\author[18]{F.~Pajot}
\author[12,13]{A.~Passerini}
\author[17]{H.~Pastoriza}
\author[2]{A.~Pelosi}
\author[3]{C.~Perbost}
\author[2]{M.~Perciballi}
\author[6,7]{F.~Pezzotta}
\author[14]{G.~Pisano}
\author[16]{M.~Platino}
\author[1,31]{G.~Polenta}
\author[3]{D.~Pr\a^{e}le}
\author[32]{R.~Puddu}
\author[18]{D.~Rambaud}
\author[33]{E.~Rasztocky}
\author[15]{P.~Ringegni}
\author[33]{G.E.~Romero}
\author[16]{J.M.~Salum}
\author[26,27]{C.G.~Sc\a'{o}ccola}
\author[8,34]{S.~Scully}
\author[12]{S.~Spinelli}
\author[3]{G.~Stankowiak}
\author[3]{M.~Stolpovskiy}
\author[16]{A.D.~Supanitsky}
\author[35]{P.~Timbie}
\author[6,7]{M.~Tomasi}
\author[14]{C.~Tucker}
\author[36]{G.~Tucker}
\author[6,7]{D.~Vigan\a`{o}}
\author[23]{N.~Vittorio}
\author[4]{F.~Wicek}
\author[5]{M.~Wright}
\author[2]{and A.~Zullo}


\affiliation[25]{University of Surrey, UK}
\affiliation[1]{Universit\a`{a} di Roma - La Sapienza, Roma, Italy}
\affiliation[32]{Pontificia Universidad Catolica de Chile, Chile}
\affiliation[36]{Brown University, Providence, USA}
\affiliation[13]{INFN sezione di Milano - Bicocca, 20216 Milano, Italy}
\affiliation[5]{University of Manchester, UK}
\affiliation[16]{Instituto de Tecnolog\a'{i}as en Detecci\a'{o}n y Astropart\a'{i}culas  (CNEA, CONICET, UNSAM), Argentina}
\affiliation[27]{CONICET, Argentina}
\affiliation[6]{Universit\a`{a} degli studi di Milano, Milano, Italy}
\affiliation[12]{Universit\a`{a} di Milano - Bicocca, Milano, Italy}
\affiliation[14]{Cardiff University, UK}
\affiliation[3]{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France}
\affiliation[31]{Italian Space Agency, Roma, Italy}
\affiliation[2]{INFN sezione di Roma, 00185 Roma, Italy}
\affiliation[10]{INFN sezione di Pisa, 56127 Pisa, Italy}
\affiliation[24]{INFN sezione di Roma2, 00133 Roma, Italy}
\affiliation[22]{University of Richmond, Richmond, USA}
\affiliation[15]{GEMA (Universidad Nacional de La Plata), Argentina}
\affiliation[9]{California Institute of Technology, USA}
\affiliation[20]{Centre de Nanosciences et de Nanotechnologies, Orsay, France}
\affiliation[30]{Institut d'Astrophysique Spatiale, Orsay (CNRS-INSU), France}
\affiliation[23]{Universit\a`{a} di Roma ``Tor Vergata'', Roma, Italy}
\affiliation[26]{Facultad de Ciencias Astron\a'{o}micas y Geof\a'{i}sicas (Universidad Nacional de La Plata), Argentina}
\affiliation[33]{Instituto Argentino de Radioastronom\a'{i}a (CONICET, CIC, UNLP), Argentina}
\affiliation[29]{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affiliation[8]{National University of Ireland, Maynooth, Ireland}
\affiliation[19]{Department of Physics, University of Oxford, UK}
\affiliation[18]{Institut de Recherche en Astrophysique et Plan\a'{e}tologie, Toulouse (CNRS-INSU), France}
\affiliation[7]{INFN sezione di Milano, 20133 Milano, Italy}
\affiliation[35]{University of Wisconsin, Madison, USA}
\affiliation[28]{Escuela de Ciencia y Tecnolog\a'{i}a (UNSAM) and Centro At\a'{o}mico Constituyentes (CNEA), Argentina}
\affiliation[17]{Centro At\a'{o}mico Bariloche and Instituto Balseiro (CNEA), Argentina}
\affiliation[21]{Centro At\a'{o}mico Constituyentes (CNEA), Argentina}
\affiliation[11]{Observatoire de Paris, Universit\'e Paris Science et Lettres, F-75014 Paris, France}
\affiliation[34]{Institute of Technology, Carlow, Ireland}
\affiliation[4]{Laboratoire de Physique des 2 Infinis Ir\a`{e}ne Joliot-Curie (CNRS-IN2P3, Universit\a'e Paris-Saclay), France}

\emailAdd{silvia.masi@roma1.infn.it}
